Model-checking lock-sharing systems against regular constraints

We study the verification of distributed systems where processes are finite automata with access to a shared pool of locks. We consider objectives that are boolean combinations of local regular constraints. We show that the problem, PSPACE-complete in general, falls in NP with the right assumptions on the system. We use restrictions on the number of locks a process can access and the order in which locks can be released. We provide tight complexity bounds, as well as a subcase of interest that can be solved in PTIME.

==> Nested-app.tex <==
\section{Proof of Lemma~\ref{lem:DELA-pat-nested}}
\label{sec:app-nested}

\DELANested*

\begin{proof}
Let $\Pat = (\OwnsN_{p}, \leq_p, \InfN_p)$.
We set $\OwnsN_{p} = \set{t_1, \ldots, t_k}$ so that $t_1 \leq_p \cdots \leq_p t_k$.

We define the automaton $\aut^p_{\Pat} = (S^p_{\Pat}, \Sigma_p \cup \set{\dummy}, \Delta^p_{\Pat}, init^p_{\Pat}, \phi^p_{\Pat})$ as follows:
If there exist $t, t'$ such that $t \in \InfN_p$, $t'\notin \InfN_p$ and $t \leq_p t'$ then no run can match this "stair pattern", hence we simply set $\aut^p_{\Pat}$ as an automaton with an empty language. From now on we will assume that it is not the case.

The states of the automaton are $S^p_{\Pat} = \set{0,\ldots,k, \infty} \times (T_p \cup \set{neutral})$, with $init^p_{\Pat} = (0,neutral)$.

\paragraph{Intuition} The first component of each state gives an index $i$ such that the run read so far is of the form $\run_0 a_1 \run_1 \cdots a_i \run_i$ with $\run_j$ "neutral" for all $j < i$, and for all $j \leq i$ $op(a_j) = \get{t_j}$ and all locks $t'$ used after $a_j$ are such that $t_j  \leq_p t'$. If the first component is $\infty$ it means we will only use locks of $\InfN_p$ in the future.

The second component of a state $(i, x)$ indicates which lock apart from $\set{t_1, \ldots, t_i}$ we acquired earliest among the ones we own. If we released all locks acquired since we took $t_i$, then the second component is $neutral$.
We do not need to keep track of all locks acquired as we are only interested in "nested" runs: If we are in state $(i,neutral)$ and acquire some lock $t$, we go to state $(i,t)$ to wait for it to be released: if we stay in state $(i,t)$ indefinitely the run is not accepted, otherwise $t$ is released we know that if the run we read is "nested" then all locks taken since we took $t$ have been released before.


\paragraph{Formal proof:}
For each action $a \in \Sigma_p \cup \set{\dummy}$ and state $s \in S^p_{\Pat}$ we have the following
transitions:
\begin{itemize}
\item If $s=(i,neutral)$ with $i < k$ then:
\begin{itemize}
	\item If $op(a) = \get{t_{i+1}}$ then $\Delta^p_{\Pat}(s,a) = \set{(i+1, neutral), (i,t_{i+1})}$
	
	\item If $op(a) = \get{t}$ with $t_i \leq_p t$ then  $\Delta^p_{\Pat}(s,a) = \set{(i,t)}$
\end{itemize}


\item If  $s=(k,neutral)$ then:
\begin{itemize}
	\item If $op(a) = \get{t}$ with $t_k \leq t$ then $\Delta^p_{\Pat}(s,a) = \set{(k, t)}$
\end{itemize}

\item If  $s=(i,t)$ with $i \leq k$ then:
\begin{itemize}
	\item If $op(a) = \rel{t}$ then $\Delta^p_{\Pat}(s,a) = \set{(i, neutral)}$
	
	\item If $op(a) = \get{t'}$ or $\rel{t'}$ with $t_i \leq_p t'$ and $t' \neq t_i$ then  $\Delta^p_{\Pat}(s,a) = \set{s}$
\end{itemize}

\item If  $s=(\infty,neutral)$ then:
\begin{itemize}
	\item If $op(a) = \get{t}$ with $t\in \InfN_p$ then $\Delta^p_{\Pat}(s,a) = \set{(\infty, t)}$
\end{itemize}

\item If  $s=(\infty,t)$ then:
\begin{itemize}
	\item If $op(a) = \rel{t}$ then $\Delta^p_{\Pat}(s,a) = \set{(\infty, neutral)}$
	
	\item If $op(a) = \get{t'}$ or $\rel{t'}$ with $t' \in \InfN_p$ then $\Delta^p_{\Pat}(s,a) = \set{s}$
\end{itemize}

\item If $op(a) = \nop$ then $\Delta^p_{\Pat}(s,a) = \set{s}$ for all $s$.

\item If $a = \dummy$ then $\Delta^p_{\Pat}((k,neutral),a) = \Delta^p_{\Pat}((\infty,neutral),a) = \set{(\infty, neutral)}$

\item Otherwise $\Delta^p_{\Pat}(s,a) = \es$.

\item We add an $\epsilon$-transition from $(k, neutral)$ to $(\infty, neutral)$. It can be eliminated by adding a few transitions to the automaton, but we allow it as it simplifies the proof.

\end{itemize}

The acceptance condition $\phi_{\Pat}$ is simply $\varinf_{(\infty,neutral)}$.

Let $\run$ be a local run of $p$ matching the given "stair pattern" $\Pat$, and let  $\run=\run_{0} a_{1} \cdots \run_{k-1} a_{k} \run_{k} \run_{k+1} \cdots$ be its "stair decomposition".
For all $i < k$ there is a path in the automaton reading $\run_{p,i}$ from state $(i, neutral)$ to itself: every letter acquiring some $t$ (thus getting to state $(i,t)$) is later followed by one releasing it. Letters using a lock lower than $t_i$ for $\leq_p$ cannot appear in $\run_{p,i}$ as otherwise $\run_p$ would not match $\Pat$. 
Furthermore, there are no $\dummy$ in $\run_{p,i}$. As a result, when $t$ is eventually released we are still in state $(i, t)$ and we go back to state $(i, neutral)$.

As a result, the run $\run_{0} a_{1} \cdots \run_{k-1} a_{k} \run_k$ labels a path from $(0, neutral)$ to $(k,neutral)$ in the automaton. 
Then all letters that appear in the $\run_i$ for $i \geq k$ are greater than $t_k$, otherwise $\run_p$ would not match $\Pat$. If $\run_p$ is finite then all the following letters are $\dummy$, and we stay in $(\infty, neutral)$ forever.

If $\run_p$ is infinite then by definition of the "stair decomposition" all the following letters use locks of $\InfN_p$ or apply $\nop$. Then we can take the $\epsilon$ transition to $(\infty,neutral)$. Each $w_{j}$ with $j \geq i+1$ labels a path from $(\infty, neutral)$ to itself: all $\get{t}$ operations that get the run to $(\infty,t)$ are matched by a later operation $\rel{t}$ taking it back to $(\infty, neutral)$. 
In both cases the run is accepting as it visits $(\infty,neutral)$ infinitely many times.

Now let $\run$ be a "nested" local run of $p$ such that $\pad{\run}$ is accepted by $\aut_{\Pat}$. Then we consider an accepting computation of $\run$ in $\aut$ and decompose $\run$ as $\run=\run_{0} a_{1} \cdots \run_{k-1} a_{k} \run_{\infty}$ with $a_i$ the first letter in the run such that the computation gets to $(i,neutral)$ after reading the prefix $\run_{0} a_{1} \cdots \run_{i-1} a_{i}$.
By definition of the automaton, we must have $op(a_i) = \get{t_i}$ for all $i$, and all operations executed after $a_i$ must be on locks greater than $t_i$ for $\leq_p$.


We show that for all $i \in \set{0,\ldots,k, \infty}$, any "nested" run labelling a path from $(i, neutral)$ to itself must be "neutral":
Suppose it is not the case, let $u$ be a "nested" run that is not "neutral" labelling a path from $(i,neutral)$ to itself, of minimal size.
The first operation on locks in $u$ must be a $\get{t}$, as otherwise $u$ cannot be read from $(i, neutral)$. In order to go back to $(i, neutral)$, there must be a later operation $\rel{t}$ in $u$. Hence, as $u$ is "nested", we have $u = a v b u'$ with $op(a) = \get{t}$, $op(b) = \rel{t}$, $v$ "neutral", and $u'$ labelling a path from $(i,neutral)$ to itself. By minimality of $u$, $u'$ must be "neutral", hence so must be $u$: contradiction.

All runs $\run_i$ label a path from $(i, neutral)$ to itself, thus they must be "neutral".

If $\run$ is finite, then so is $\run_{\infty}$. Furthermore $\run_{\infty}$ is "neutral" as it must label a path from $(k,neutral)$ to itself. Thus $\run$ must match the "stair pattern" $\Pat$.

Otherwise, we cut $\run_{\infty}$ in parts so that  $\run_{\infty}= \run_k \run_{k+1} \cdots$ with $\run_k$ labelling a path from $(k, neutral)$ to itself and for all $j \geq k+1$, $\run_j$ labelling a path from $(\infty,neutral)$ to itself. 

This decomposition exists as, for $\run$ to be accepted, $\run_{\infty}$ must label a path starting in $(k, neutral)$, taking at some point the $\epsilon$ transition from $(k, neutral)$ to $(\infty, neutral)$, and then going back infinitely many times to $(\infty, neutral)$.

As each $\run_j$ labels a path from either $(k, neutral)$ or $(\infty,neutral)$ to itself, they are all "neutral". Furthermore, the $\run_j$ with $j \geq k+1$ can only use locks of $\InfN_p$, as the automaton only allows those operations from states with an $\infty$ first component.

As a result, $\run$ matches pattern $\Pat$. 
\end{proof}

==> Pattern_characterization.tex <==
\section{Proof of Proposition~\ref{prop:charac-schedulable-pat}}
\label{app:pat-charac}

\CHARACPATTERNS*

\begin{proof}
	{\Large \textbf{$\Rightarrow$:}} We start with the left-to-right implication. Let $(\run_p)_{p \in \Proc}$ be a family of local runs, 
	suppose they can be scheduled into a "process-fair" global run $\run$.
	
	For all finite local runs $\run_p$, as $\run$ is "process-fair", 
	after some point $p$ cannot ever execute any action.
	
	As a consequence, $s_p$ (the state reached after executing $\run_p$) cannot have any outgoing
	transition executing $\rel{}$ or $\nop$, as those can always be executed.  
	The locks of $\Blocks_p$ are never free after some point, as otherwise $p$
	would be enabled infinitely often on the run, so the run would not be
	"process-fair". 
	This shows condition~\ref{C1}.
	
	%		If $u$ is finite then it leads to a "global deadlock". 
	%		In that case, by the characterization of "global deadlocks" 
	%		(see~\cite{GimMMW22}), 	all conditions are met.
	%		
	%		If $u$ is infinite, then let $\dashover{\Inf_p}$ be the "pattern" of $\run_p$ for 
	%		all infinite $\run_p$. 
	All finite runs $\run_p$ stop while holding the locks of $\Owns(\run_p)$.
	All infinite $\run_p$ eventually acquire and never release the locks 
	of their $\Owns(\run_p)$.
	Hence the $\Owns(\run_p)$ sets need to be pairwise disjoint, proving condition~\ref{C3}.
	
	Furthermore, if a lock is not in some $\Owns(\run_p)$ then 
	it is free infinitely often, 
	and thus cannot be in $\Blocks_p$ for any $p$, as $\run$ is "process-fair".
	This proves condition~\ref{C4}.
	
	All locks of $\bigcup_{J \in \Inf(\run_q)} J$ are held by $q$ infinitely often, hence they cannot be in any $\Owns(\run_p)$ with $p \neq q$, which shows 
	condition~\ref{C5}.
	
	If a run $\run_p$ of a process $p$ using locks $t_1,t_2$ has a "pattern"
	$\fillover{\set{t_1}}$ or $\fillover{\set{\set{t_1}}}$ 
	then the last operation on $t_1$ (when $p$ acquires it for the last time) is followed by at least 
	one operation on $t_2$ in the run $\run$. 
	We satisfy condition~\ref{C6} by setting $\leq$ as an order on locks 
	such that $t \leq t'$ whenever $t$ is only acquired finitely many times and there is an operation on $t'$ 
	after the last operation on $t$ in $\run$ .
	
	We demonstrate condition~\ref{C7} by contradiction.
	Say there exist such locks and process, i.e., there exist $t = t_1, \ldots, t_n = t'$ and $p_1, \ldots, p_{n-1}$ without $p$ such that 
	for all $1 \leq i < n$, $p_i$ accesses $t_i$ and $t_{i+1}$ 
	and $\run_{p_i}$ is "switching". 
	Then all $p_i$ are always holding a lock after some point.
	
	As $\set{t_n, t_1} \in \Inf(\run_p)$, this means that $p$ holds $t_n$ and $t_1$ 
	simultaneously infinitely often. 
	Whenever that happens, processes $p_1,\dots,p_{n-1}$ have to share the remaining 
	($n-2$) locks, hence one of them holds no lock, 
	contradicting the fact that $\emptyset \notin \Inf(\run_{p_i})$ for all $i$.
	
	{\Large \textbf{$\Leftarrow$:}} For the other direction, 
	suppose $(\run_p)_{p \in \Proc}$ satisfies all the conditions of the list.
	We construct a "process-fair" global run 
	whose local projections are the $\run_p$.
	
	To do so, we will construct a sequence of finite runs $v_0, v_1, \ldots$ such that $v_0 v_1 \cdots$ is such a global run.
	
	We will ensure that the following property is satisfied for all $i \in \nats$:
	
	\begin{align}\label{prop-vi}\nonumber
		& \text{For all processes } p, \text{ after executing } v_0\cdots v_i,\\
		& \text{ if } \Owns(\run_p) \in \Inf(\run_p) \text{ then }  \Owns((v_0\cdots v_i)|_p) = \Owns(\run_p)\\
		&\nonumber \text{ otherwise } w_p \text{ is "switching" and } p \text{ holds one lock.}
	\end{align}

	We will also make sure that all $p$ with an infinite $\run_p$ execute an action in infinitely many $v_i$.
	
	The first run $v_0$ has to be constructed separately as we require it to satisfy some extra conditions.
	We construct $v_0$ such that for all $p$: 
	\begin{itemize}
		\item If $\run_p$ is finite then $v_0|_p = \run_p$.
		
		\item If $\run_p$ is infinite then $\run_p = v_0|_p u_p$ 
		with $u_p$ such that for every prefix $u'_p$ of $u_p$, $\Owns(v_0|_p u'_p) \in \Inf(\run_p)$.
		Furthermore if $\emptyset \in \Inf(\run_p)$ then $\Owns(v_0|_p) = \emptyset$.
		
		In other words, we execute a prefix of each infinite run 
		such that what follows matches its asymptotic behaviour.
	\end{itemize}
	
	\paragraph{Construction of $v_0$} 	
	\begin{itemize}
		\item First, for all infinite $\run_p$ such that $\emptyset \in \Inf(\run_p)$, 
		there exist arbitrarily large finite prefixes of $\run_p$ 
		ending with $p$ having no lock. 
		Hence we can select one of those prefixes $v_0|_p$, 
		large enough for $p$ to never hold a set of locks 
		not in $\Inf(\run_p)$ later in the run.
		We execute all such $v_0|_p$ at the start. All locks are free afterwards.
		
		\item We then execute for all other $p$ with "weak patterns", 
		their maximal prefix ending with $p$ having no lock.
		All locks are still free.
		
		
		\item Then we execute all $\run_p$ with "strong patterns", 
		in increasing order according to $\leq$ (see condition~\ref{C6}) 
		on the locks $t_p$ such that $\Owns(\run_p)=\set{t_p}$. 
		We execute in full the finite ones, while for the infinite ones 
		we execute a prefix $v_0|_p$ such that in the end $p$ owns only $t_p$ and 
		never acquires the other lock afterwards (recall that $\Inf(\run_p) = \set{\set{t_p}}$ in that case).
		Say we executed some of those local runs, let $p$ be a process such that $\run_p$ has a "strong 
		pattern" accessing locks $t_1 \leq t_2$, say we want to execute $v_0|_p$. 
		By condition~\ref{C3}, all $\Owns(\run_p)$ are disjoint, hence there is no other 
		process $q$ with $\Owns(\run_q) = \set{t_1}$.
		The only locks that are not free at that point are the $t$ such that 
		$t < t_1$ and $\Owns(\run_q) = \set{t}$ for some $q$ with a "strong pattern".
		Therefore, both $t_1$ and $t_2$ are free, and $v_0|_p$ can be executed.
		In the end the aforementioned locks $t_p$ are taken and all others are free.
		

		
		\item  	Then we consider the finite $\run_p$ with non-empty $\Owns(\run_p)$ and "weak patterns". 
		For those, we can execute the rest of the run 
		(we already executed the maximal prefix leading to them holding no lock), 
		as all they do is take the locks in $\Owns(\run_p)$, 
		which are free by conditions~\ref{C3} and \ref{C5}.
		
		\item 	For the infinite $\run_p$ with non-empty $\Owns(\run_p)$ and "weak patterns", there are two possibilities: 
		
		\begin{itemize}
			\item The first is that $p$ eventually keeps the same set of locks forever 
			and never executes any more operations on locks. 
			Then its "trace" $\trace{\run_p}$ is of the form 
			either $(\pow{T_p})^* \emptyset \set{t_1}^\omega$ 
			or $(\pow{T_p})^*\set{t_1,t_2}^\omega$. 
			In that case clearly we can just execute the run until we reach a point 
			after which $p$ only ever owns $\Owns(\run_p)$ forever.
			We can do this as all locks taken so far are either in $\Owns(\run_q)$ 
			for some $q$ with finite $\run_q$ 
			or are in an element of some $\Inf(\run_q)$ for some $q$.
			Thus all locks from those $\Owns(\run_p)$ are free 
			by conditions~\ref{C3} and \ref{C5}.
			
			\item The other possibility is that 
			$\trace{\run_p} \in (\pow{T_p})^*(\set{t_1}^* \set{t_1, t_2})^\omega$ 
			with $\set{t_1, t_2} = T_p$ and $\Owns(\run_p) = \set{t_1}$. 
			This happens if $p$ ultimately holds one lock forever 
			and acquires and releases the other one infinitely many times.
			At that point all locks that are taken are in some $\Owns(\run_p)$, thus by condition \ref{C5} both locks of $p$ are free. 
			Hence we can execute enough steps of $\run_p$ to reach a point at which 
			$p$ holds only $t_1$ and will only hold sets of locks of $\Inf(\run_p)$ afterwards.
		\end{itemize}
		
		
		\item Finally we consider the infinite "switching" runs $\run_p$. 
		All those processes must have $T_p \in \Inf(\run_p)$, hence by condition \ref{C5} 
		all their locks are free.
		By condition \ref{C7}, $\Ginf$ is acyclic.
		We can therefore pick one of those processes $p$ and a lock $t$ such that 
		no other such process accesses $t$. 
		We execute $\run_p$ until 
		$p$ only owns $t$ will only own sets of locks of $\Inf(\run_p)$ afterwards.
		All locks of the other such $p$ are still free, hence we can iterate that step until we executed a prefix of each of those $p$.
	\end{itemize}
	
	
	We have constructed a finite run $v_0$ whose projection $v_0|_p$ on $\S_p$ is such that if $\run_p$ is finite then $\run_p = v_0|_p$ 
	and  if $\run_{p}$ is infinite then $v_0|_p$ is a prefix of $\run_p$ such that all local configurations seen later in the run are in $\Inf(\run_p)$. Moreover $v_0$ satisfies property~\ref{prop-vi}.
	
	We now construct the remaining parts of the run.
	If all $\run_p$ are finite then $v_0$ proves the lemma (we can set all other $v_i$ as $\epsilon$). Otherwise we must describe the rest of the "process-fair" global run whose projections are the $\run_p$.	
	We start with a small construction that will help us define the $v_i$.	
	
	Suppose we constructed $v_0, \ldots, v_i$ so that property~\ref{prop-vi} is satisfied for all $j \leq i$. 
	Now suppose some lock $t_0$ is not in any $\Owns(\run_p)$ 
	and is not free after executing $v_0 \cdots v_i$.
	Then there exists a "switching" run $\run_{p_1}$ with $t_0 \in T_{p_1}$.
	
	Let $t_1$ be the other lock of $p_1$, 
	say it is not free. 
	By property~\ref{prop-vi}, $p_1$ holds only one lock and thus does not hold $t_1$. 
	By condition~\ref{C5} $t_1$ cannot be in some $\Owns(\run_p)$, thus, again by property~\ref{prop-vi}, as $t_1$ is not free,
	there exists a "switching" $\run_{p_2}$ such that $t_1 \in T_{p_2}$.
	Let $t_2$ be the other lock of $p_2$.
	
	We construct this way a sequence of processes $p_1, p_2, \ldots$ 
	and of locks $t_0, t_1, \ldots$ such that 
	$T_{p_j} = \set{t_{j-1}, t_{j}}$ and $\run_{p_j}$ is "switching" for all $j$. 
	This sequence cannot be infinite as each $p_j$ labels an edge in $\Ginf$, 
	which is finite and acyclic.
	
	Hence there exists $k$ such that $t_k$ is free. 
	We can therefore execute $\run_{p_k}$ until $p_k$ holds $t_k$
	and not $t_{k-1}$, then execute $\run_{p_{k-1}}$ 
	until $p_{k-1}$ holds $t_{k-1}$ and not $t_{k-2}$, and so on
	until $t_1$ is free.
	
	Hence if a lock $t$ is not in any $\Owns(\run_p)$ but is not free 
	after executing $v_0 \cdots v_i$ then we can prolong the prefix run 
	so that $t$ is free and some lock from the same connected component 
	in $\Ginf$ is not. 
	For all such $t$ and $i$ we name this prolongation of the run $\pi_{t,i}$.
	
	Say we already constructed $v_0, \ldots, v_i$, and that property~\ref{prop-vi} is satisfied for all $j \leq i$. We construct $v_{i+1}$. 
	Let $p$ be either a process that never executed an action, 
	or if there are no such processes, 
	the process whose last action in $v_0\cdots v_i$ is the earliest.
	
	We prolong the current run so as to execute some actions of $\run_p$.
	If the next action of $\run_p$ applies an operation $\nop$ we can execute it right away.
	The next action cannot execute a $\rel{}$ operation:
	After executing $v_0$ all processes with infinite $\run_p$ only own sets of locks of $\Inf(\run_p)$.
	By property~\ref{prop-vi}, if $\run_p$ is "switching" then after executing $v_0\cdots v_i$ the process $p$ holds one lock and will not release it as it would be left with no lock and $\es \notin \Inf(\run_p)$. If $p$ is not "switching" then after executing $v_0\cdots v_i$ it holds $\Owns(\run_p)$ and cannot release any lock as it keeps those forever. 
	
	Hence we are left with the case where the next action of $p$ acquires a lock $t$.
	If $t$ is not free we apply $\pi_{t,i}$ to free it 
	(and block another lock of the same connected component of $\Ginf$). 
	Note that after executing $\pi_{t,i}$ all processes with "switching" runs still hold one lock, and the others have not moved.
	
	\begin{itemize}
		\item 	If $\run_p$ is "switching" then $p$ was already holding a lock $t'$, and it can then take $t$ and then run $\run_p$ until it holds only 
		one lock again, thus respecting property~\ref{prop-vi}.
		
		\item Otherwise $p$ was holding $\Owns(\run_p)$ (by Property~\ref{prop-vi}) 
		and we have to let him take $t$ and then continue
		until $p$ holds exactly $\Owns(\run_p)$ again.
		
		\begin{itemize}
			\item If we can do it right away we do so.
			
			\item Otherwise it means that $p$ needs its other lock $t'$ to reach that 
			next step, and that this lock is taken. 
			More precisely, it means that $\Owns(\run_p) = \emptyset$ and 
			$\emptyset, \set{t,t'} \in \Inf(\run_p)$.
			
			As $\set{t,t'} \in \Inf(\run_p)$, by condition~\ref{C7},
			$t$ and $t'$ are not in the same connected component of $\Ginf$. 
			Hence we can execute $\pi_{t',i}$, without locking $t$ back, as $\pi_{t,i}$ and $\pi_{t',i}$ use disjoint sets of locks and processes.
			
			This ensures that both $t$ and $t'$ are free, 
			which allows $p$ to take $t$ and proceed to the next point 
			at which it holds $\emptyset$.
		\end{itemize}
		In both cases we end up in a configuration where $p$ owns $\Owns_{p}$, all processes with "switching" runs hold exactly one lock, and the other processes did not move, thus respecting property~\ref{prop-vi}. 
	\end{itemize}
	
	
	We have constructed $v_{i+1}$, ensuring that property~\ref{prop-vi} is satisfied for $i+1$. 
	Furthermore $v_{i+1}|_p$ is non-empty for $p$ a process with infinite $\run_p$ which either never executed anything before or executed its last action the earliest. This ensures that all $p$ with infinite $\run_p$ execute infinitely many actions in $v_0 v_1 \cdots$.
	Hence we obtain a global run $v = v_0 v_1 \cdots$ such that for all $p$ we have $v|_p = \run_p$.
	
	Furthermore we ensured that $v$ is "process-fair" as all $p$ 
	with finite runs are blocked: 
	all such $\run_p$ lead to a state from which only locks of $\Blocks_p$ can be taken, by condition~\ref{C1}, 
	and by condition~\ref{C4} all $\Blocks_p$ are included in 
	$\bigcup_{p \in \Proc} \Owns(\run_p)$, 
	the set of locks that are never free from some point on.
	
	As a result, there exists a "process-fair" run 
	whose local projections are the $\run_p$, 
	proving the right-to-left implication.
\end{proof}

==> Pspaceproof.tex <==
\section{Proof of Proposition~\ref{prop:PSPACE-LSS}}
\label{app:pspace-lss}

\PSPACELSS*

	The \PSPACE~upper bound is easy to obtain: It suffices to guess a state $s_p$ in each $\aut_p$ and $s'_p$ in each $\objaut{p}$, and then guess a sequence of letters in $\S$ while keeping track of the states reached by that sequence in the $\aut_p$ and $\objaut{p}$. 
	
	If we reach a configuration with each $\aut_p$ in state $s_p$ and each $\objaut{p}$ in $s'_p$, we start memorising the set of visited states in each $\objaut{p}$. 
	If we reach that configuration again, we stop and accept if and only if the set of visited states in the $\objaut{p}$ satisfies $\phi$.
	This comes down to guessing an ultimately periodic run in the global system and checking that it satisfies the objective.
	
	The difficulty is to obtain the \PSPACE-hardness with a fixed number of locks per process. To do so we reduce the emptiness problem for the intersection of a set of deterministic automata. 
	
	Without loss of generality we will assume that there are at least two automata, that they are all over alphabet $\set{0,1}$, and that their languages are all included in $11(00+01)^*$: we can always apply a small transformation to each automaton so that, if its language was $\mathcal{L}$, it becomes $11 h(\mathcal{L})$ with $h$ the morphism mapping $0$ to $00$ and $1$ to $01$. The intersection of those languages is empty if and only if the intersection of the original languages was empty.
	
	Let $\aut_1, \cdots, \aut_n$ (with $n \geq 2$) be automata, with, for each $1 \leq i \leq n$, $\aut_i = (S_i, \set{0,1}, \delta_i, init_i, F_i)$.
	We construct a "sound" "exclusive" "LSS" $\tss$ as follows:
	
	For each $1 \leq i \leq n$ we have a process $p_i$ which is in charge of simulating $\aut_i$.	
	The set of locks is $T = \set{0_i, 1_i, key_i \mid 1 \leq i \leq n}$.
	For all $i$, $p_i$ accesses locks $0_i, 1_i, key_i$, as well as $0_{i+1}, 1_{i+1}, key_{i+1}$ if $i \leq n-1$ and $0_{1}, 1_1$ if $i =n$. Thus a process uses at most 6 locks in total.
	
	For all $1 \leq i \leq n$ and $t$ accessed by $p_i$, we have two actions $\get{t}^i$ and $\rel{t}^i$, with which $p_i$ acquires and releases lock $t$, as well as actions $\nop^i$ and $end^i$ with no effect on locks.
	
	In the proof the following local sequences will be important:
	
	\[\send(0) = \rel{0_n}^n \get{0_{0}}^n \rel{1_n}^n \get{1_0}^n \rel{0_{0}}^n \get{0_n}^n \rel{1_{0}}^n \get{1_n}^n\]
	
	\[\rec_i(0) = \nop^i \get{0_{i+1}}^i \rel{0_{i}}^i \get{1_{i+1}}^i \rel{1_{i}}^i \get{0_{i}}^i \rel{0_{i+1}}^i \get{1_{i}}^i \rel{1_{i+1}}^i\]
	
	
	$\send(1)$ and $\rec_i(1)$ are defined analogously, by replacing $0$ by $1$ and $1$ by $0$ everywhere.
	
	The following global sequences will be useful as well:
	
	\[ \acqs(0) = \get{0_{n}}^{n-1}\rel{0_{n-1}}^{n-1} \cdots  \get{0_{1}}^{1}\rel{0_{0}}^{1}\]
	
	\[ \rels(0) = \get{0_{0}}^{1}\rel{0_{1}}^{1} \cdots  \get{0_{n-1}}^{n-1}\rel{0_{n}}^{n-1}\]
	
	\[ \NOP = \nop^{1} \cdots  \nop^{n-1}\]
	
	$\acqs(1)$ and $\rels(1)$ are defined analogously, by replacing $0$ by $1$ and $1$ by $0$ everywhere.	
	
	The transition system of each process $p_i$ is designed as follows: 
	We start with $\aut_i$, and we replace every transition labelled $0$ with a sequence of transitions labelled by actions of $\send(0)$ if $i=n$, and $\rec_i(0)$ if $1 \leq i \leq n-1$ (there is at least one such $i$ as $n \geq 2$).
	
	Furthermore we add a few transitions so that each $p_i$ with $i \leq n-1$ executes $\start_i = \get{key_{i+1}}^i \get{0_i}^i \get{1_i}^i  \get{key_i}^i \rel{key_{i+1}}^i$ before entering the initial state of $\aut_i$.
	If $i=n$ that sequence is $\start_n = \get{a_n}^n \get{b_n}^n \get{key_n}^n$.
	We also add a transition reading $end^i$ from all states of $F_i$ to a state $stop_i$ with no outgoing transition.
	
	The objective is that the action $end^i$ is executed for all $1 \leq i \leq n$.
	
	One direction is easy.
	Say there is a word $u = b_1 b_2 \cdots b_m$ in the intersection of the languages of the $\aut_i$. Then we start by executing all $\start_i$ sequences for all $i$ in increasing order, and then, for each $1 \leq j \leq m$ (in increasing order), we execute the sequence of operations 
	
	
	\begin{align*}
		seq(b_j) = &\rel{(b_j)_n}^n \NOP~\acqs(b_j) \get{(b_j)_0}^n \rel{(1-b_j)_n}^n\\ &\acqs(1-b_j) \get{(1-b_j)_0}^n \rel{(b_j)_0}^n \rels(b_j)\\ &\get{(b_j)_n}^n\rel{(1-b_j)_0}^n \rels(1-b_j) \get{(1-b_j)_n}^n 
	\end{align*}
	
	
	This run projects on $p_i$ as $\start_i \rec_i(b_1) \rec_i(b_2) \cdots \rec_(b_m)$ if $i\leq n-1$ and $\start_i \send(b_1) \send(b_2) \cdots \send(b_m)$ if $i=n$. As $u$ is in the language of $\aut_i$, $p_i$ can execute this run locally.
	It can be easily checked that all operations in that run are valid in the current configuration, hence this sequence can be executed.
	
	As $u$ is accepted by all $\aut_i$, after executing the sequence above each process $p_i$ ends up in a state of $F_i$, and thus they can all execute $end^i$ one after the other.
	
	Conversely, suppose there is some run $\run$ whose local projection $\run|_p$ on each process $p$ is ends with $end^i$.
	Each $\run|_{p_i}$ must start with the execution of $\start_i$.
	
	We prove the following lemma:
	
	\begin{lemma}
		For all $j \in \nats$, let $\run_j$ be the shortest prefix of $\run$ whose projection on $p_n$ is $\start_n \send(b_1) \cdots \send(b_j)$. 
		Then the projection of $\run_j$ on every other $p_i$ has $\rec_i(b_1) \cdots \rec_i(b_j)$ as a suffix.
	\end{lemma}

	\begin{proof}
		We prove this by induction on $j$.
		For $j=0$ it is trivial.
		Let $j \in \nats$, suppose the claim is true for $j$, we show it for $j+1$.
		
		First of all note that for all $i \geq 1$, if $p_i$ has finished executing $\start_i$ then it holds $k_i$ and will never release it, hence $p_{i-1}$ either has executed $\start_{i-1}$ in full or has not begun executing it. In the second case, $p_{i-1}$ will never be able to advance, which is impossible as $\run|_p$ is not empty. As a result, after $p_n$ has executed $\start_n$, all other $p_i$ must have executed $\start_i$.
		
		Another important remark is that after executing $\start_i$, all $p_i$ alternate between a $\get{}$ and a $\rel{}$ no matter which local run they execute. While $p_n$ starts with a $\rel{}$, all other processes start with a $\get{}$. Therefore $p_n$ always holds either 2 or 3 locks, while all others always hold either 3 or 4.
		There are $n$ processes and $3n$ locks in total, hence at all times the global configuration is such that either all locks are taken and the next operation of some process $p$ is $\rel{}$ (and $\get{}$ for all others) or one lock is free and all processes have a $\get{}$ as their next operation.
		
		Now say process $p_n$ has started executing $\send(b_{j+1})$ by releasing $(b_{j+1})_n$. This means some other process must have taken $(b_{j+1})_n$, which can only be $p_{n-1}$. The only possibility is that $p_{n-1}$ then releases $(b_{j+1})_{n-1}$, which can only be taken by $p_{n-2}$, ... We must end up executing $\acqs(b_{j+1})$, which ends with $(b_{j+1})_0$ free, which can only be taken by $p_n$.
		
		By continuing this reasoning we conclude that $\run_{j+1}=\run_j seq(b_{j+1})$, proving the lemma.
	\end{proof}

As all $p_i$ execute $end_i$ in $\run$, in particular $\run|_{p_n}$ ends with $end^n$, hence it is necessarily of the form $\start_n \send(b_1) \cdots \send(b_m) end^n$. 
Let $\run'$ be $\run$ where all $end^i$ have been erased.
The lemma above allows us to conclude that for all $i$, $\run'|_{p_i}$ has $\rec_i(b_1)  \cdots \rec_i(b_m)$ as a suffix. 

Recall that the languages of all $\aut_i$ are included in $11(00+01)^*$.
Moreover, we know that $b_1 \cdots b_m$ is in the language of $\aut_{n}$,
hence $b_1 = b_2 =1$. Furthermore, all $\run'|_{p_i}$ ($i<n$) are of the form $\start_i \rec_i(x_1) \cdots \rec_i(x_r)$ with $x_1 \cdots x_r$ in the language of $\aut_i$.
As the only moment a factor $11$ can appear in a word of those languages is at the beginning, for $\run'|_{p_i}$ to have $\rec_i(b_1) \cdots \rec_i(b_m)$ as a suffix, we must have $\run'|_{p_i} = \start_i \rec_i(b_1) \cdots \rec_i(b_m)$. 

As a consequence, for all $i$ we have $\run|_{p_i} = \start_i \rec_i(b_1) \cdots \rec_i(b_m) end^i$ and thus $b_1 \cdots b_m$ must be accepted by all $\aut_i$.

We have proven that this system had a run in which each $p_i$ reads $end^i$ if and only if there is a word accepted by all $\aut_i$.

As that condition is easily expressible as a "regular objective", we obtain the \PSPACE-hardness of the "regular verification problem" for "sound" "exclusive" "LSS" with 6 locks per process.
However, our goal was to prove the \PSPACE-hardness of the "process deadlock problem" for "sound" "exclusive" "LSS".

To do so, we add a process $q$ and locks $\ell_{i}$ for $1 \leq i \leq n+1$ so that the transition system of $q$ simply takes $\ell_{n}$ and then goes to a state with a self-loop executing $\nop$. We also add, for each $1 \leq i \leq n$, a sequence of transitions from $stop_i$ which take $\ell_i$, then $\ell_{i-1}$ and release $\ell_i$ if $i \geq 2$, and simply take $\ell_i$ if $i=1$, to end up in a state with no outgoing transition.

We show that there is a "process-fair" run with a finite projection on $q$ if and only if there is one in the previous "LSS" such that each $p_i$ executes $end_i$.

If the latter is true, then we just take the same run and prolong it so that each $p_i$ takes $\ell_i$. Then all $\ell_i$ are taken, and all processes need some $\ell_i$ to advance, we have reached a global deadlock (in particular the run is "process-fair", and its projection on $q$ is finite).

Conversely, suppose we have a "process-fair" run in the new "LSS" with a finite projection on $q$. Then $q$ must be blocked, which is only possible if $\ell_n$ is held forever by $p_n$, which in turn is only possible if $\ell_{n-1}$ is held forever by $p_{n-1}$... We conclude that all $p_i$ must be holding $\ell_i$ forever from some point on, and thus that they all read $end_i$.

We project that run to erase all actions getting an $\ell_i$. We obtain a run of the previous system in which every process has executed $end_i$.

As a result, the new "LSS" has a "process-fair" run in which $q$ is blocked if and only if the former "LSS" has a run in which every $p_i$ has executed $end_i$, if and only if the $\aut_i$ recognise a common word.

As a result, the "process deadlock problem" is \PSPACE-complete for "sound" "exclusive" "LSS" with 8 locks per process. 

==> Ptimeproof.tex <==
\section{Proof of Proposition~\ref{prop:ptime-exclusive}}
\label{app:ptime-exclusive}

\PTIMEEXCLUSIVE*


Let $\tss$ be a "sound" "exclusive" "2LSS" and $p$ a process of $\tss$.	

\begin{lemma}\label{lem:fair-exclusive}
	Let $(s_p, B_p)_{p \in \Proc}$ be a "global configuration" and for each process $p$ let $u'_p$ be a local run starting in $(s_p, B_p)$ and such that $u'_p$ is either infinite or leads to a state with no outgoing transitions.
	
	There exists a "process-fair" global run $\run$ from $(s_p, B_p)_{p \in \Proc}$ such that for all $p$ its projection $\run_p$ on $\S_p$ is a prefix of $u'_p$.
\end{lemma}

\begin{proof}
	We construct $\run$ by iterating the following step:
	For each $p$ we set $u'_p = v_p w_p$ with $v_p$ the prefix of $u'_p$ executed so far.
	We select uniformly at random a process $p \in \Proc$. If it can execute the first action of $w_p$ then we let it do so, otherwise we do nothing.
	
	We iterate this procedure indefinitely.
	This produces a (possibly finite) global run of the system such that its local projections are prefixes of the $u'_p$. We prove that it is "process-fair".
	
	Let $p \in \Proc$, assume that $p$ has an available action at infinitely many steps.
	As our "LSS" is "exclusive", whenever $p$ has an available action and is in some state $s$,
	either all outgoing transitions are executing an operation $\nop$ or $\rel{}$ (and thus can all be executed as the system is "sound"), or they all acquire the same lock $t$ (as the system is "exclusive").
	Hence if one outgoing transition can be executed , they all can and thus in particular the next action of $u'_p$ is available.
	As a result, $p$ can execute the next action of $u_p$ at infinitely many steps, and thus will progress infinitely many times in $u_p$.
	
	In conclusion, with this procedure we either reach a "global deadlock", or we always have an available action, implying that at least one process will be able to progress infinitely many times and that the resulting run $u$ is infinite. 
	In the latter case, all processes that can execute an action at infinitely many steps of the run will do so, proving that the run is "process-fair".
\end{proof}

\begin{definition}
	Define the graph $G$ whose vertices are locks and with an edge $t_1 \edge{p} t_2$ if and only if the process $p$ has a local run $\run_p$ ending in a state where all outgoing transitions acquire $t_2$ and such that $\Owns(\run_p) = \set{t_1}$. We say that $\run_p$ ""witnesses"" the edge $t_1 \edge{p} t_2$.
\end{definition}

\begin{lemma}
	\label{lem:always-one-weak}
	For all $p \in \Proc$, if there is a $p$-labelled edge $t_1 \edge{p} t_2$ in $G$  then either $t_1 \edge{p} t_2$ is "witnessed" by a run with a weak pattern or its reverse $t_2 \edge{p} t_1$ is in $G$ and is "witnessed" by a run with a weak pattern.
\end{lemma}

\begin{proof}
	As $p$ has an edge $t_1 \edge{p} t_2$ in $G$, there is a local run which acquires both locks of $p$ at the same time. Let $\run_p$ be such a run of minimal length. The last operation in $\run_p$ must be a $\get{}$, by minimality, hence $\run_p$ is of the form $\run'_p a$ with $op(a) = \get{t}$ for some $t \in \set{t_1, t_2}$.
	Furthermore, suppose the last operation in $\run'_p$ besides $\nop$ is a $\rel{}$, then there is a previous configuration in $\run_p$ in which $p$ holds both of its locks, contradicting the minimality of $\run_p$. Hence $\run'_p$ has a weak pattern, and it leads to a state where $p$ may acquire $t$, thus has to acquire $t$ as the system is "exclusive". Furthermore $p$ is then holding its other lock, therefore $\run'_p$ "witnesses" an edge in $G$.
\end{proof}

\begin{lemma}
	\label{lem:cond-cycle}
	If $p$ has a reachable transition acquiring some lock $t$ and there is a path from $t$ to a cycle in $G$ then there is a "process-fair" global run with a finite projection on $p$. 
\end{lemma}

\begin{proof}
	Let $t = t_0 \edge{p_1} t_1 \edge{p_2} \cdots \edge{p_k} t_k$ be such a path in $G$ and let $t_k = t'_1 \edge{p'_1} \cdots t'_n \edge{p'_n} t'_{n+1} = t'_1 = t_k$ be such  a cycle.
	
	For all $1 \leq i \leq k$ we choose a run $\run_i$ "witnessing" $t_{i-1} \edge{p_i} t_i$. Similarly for all $1 \leq j \leq n$ we choose a run $\run'_j$ "witnessing" $t'_{j} \edge{p'_i} t'_{j+1}$, and we choose it so that it has a weak pattern whenever possible.
	
	\paragraph{Case 1: }If there exists $j$ such that $\run'_j$ has a weak pattern, then we proceed as follows: Let $\run'_j = u_j v_j$ so that $u_j$ is the maximal "neutral" prefix of $\run_j$. We execute $u_j$, leaving all locks free.
	Let $m$ be the maximal index such that $t_m \in \set{t'_1, \cdots, t'_n}$. We execute all $\run_i$ in increasing order for $1 \leq i \leq m$.
	
	Then we execute $\run'_{j+1} \cdots \run'_n \run'_1 \cdots \run'_{j-1}$ and then $v_j$. Then we end up in a configuration where all $p_i$ with $i\leq m$ are holding $t_{i-1}$ and need $t_i$ to advance, while all $p'_i$ are holding $t'_i$ and need $t'_{i+1}$ to advance. As $t_j \in \set{t'_1,\ldots, t'_n}$, all those processes are blocked, and in particular $t = t_0$ is held by a process which will never release it.
	
	As $p$ has a reachable transition taking $t$, we can define $\run_p$ as a shortest run that ends in a state where some outgoing transitions takes a lock of $\set{t_0, \ldots, t_m, t'_1, \ldots, t'_n}$. By minimality this run can  be executed, as all other locks are free. 
	By exclusiveness, it reaches a state where all transitions take the same non-free lock.
	
	By Lemma~\ref{lem:fair-exclusive} we can extend this run into a "process-fair" one, whose projection on $p$ can only be $\run_p$, as $p$ will never be able to advance further.
	
	\paragraph{Case 2: }Now suppose there is no $j$ such that $\run'_j$ has a weak pattern, then as we took all $\run'_j$ with weak patterns whenever possible, it means there is no local run with a weak pattern "witnessing" any of the $t'_j \edge{p'_j} t'_{j+1}$.
	We can then apply Lemma~\ref{lem:always-one-weak} to show that the reverse cycle $t'_1 = t'_{n+1} \edge{p'_n} t'_n \cdots \edge{p'_1} t'_1$ exists in $G$ and all its edges are "witnessed" by runs with weak patterns.
	Hence we can apply the arguments from the previous case using this cycle to conclude.
\end{proof}

\begin{lemma}
	\label{lem:cond-inf}
	If $p$ has a reachable transition acquiring some lock $t$ and there is a path in $G$ from $t$ to some $t'$ such that there is a process $q$ with an infinite local run $\run_q$ acquiring $t'$ and never releasing it (i.e., such that $t' \in \Owns(\run_q)$), then there is a "process-fair" global run with a finite projection on $p$. 
\end{lemma}
\begin{proof}
	Let $t = t_0 \edge{p_1} t_1 \edge{p_2} \cdots \edge{p_{k}} t_k = t'$ be the shortest path from $t$ to $t'$.
	Let $\run_p$ be a local run of $p$ acquiring $t$ at some point, either infinite or leading to a state with no outgoing transition. 
	For each $1 \leq i \leq k$ we select a local run $\run_i$ of $p_i$ "witnessing" $t_{i-1} \edge{p_i} t_i$.
	Furthermore we select those $\run_i$ with "weak patterns" whenever possible. 
	Let $t_q$ be the other lock used by $q$ besides $t'$, and let $\run_q$ be an infinite run of $q$ in which $t'$ is eventually taken and never released.
	We can decompose $\run_q$ as $u_q v_q$ where $u_q$ is the largest "neutral" prefix of $\run_q$. 
	We distinguish several cases:
	
	\paragraph{Case 1:} $t_q \notin \set{t_0, \ldots, t_k}$, or $t_q$ is not used in $v_q$. Then we can execute $u_q$, leaving all locks free, then $\run_1 \cdots \run_k$, which can be done as the execution of $\run_1 \cdots \run_i$ leaves $t_{i}, \ldots, t_k$ free and thus $\run_{i+1}$ can be executed.
	Let $v_q = v'_q v''_q$ with $v'_q$ a prefix of $v_q$ large enough so that $t'$ is held by $q$ and never released later.
	Then as no $t_i$ is used in $v_q$, we can execute $v'_q$. 
	Let $\run$ be the run constructed so far.
	Then by Lemma~\ref{lem:fair-exclusive} we can construct a "process-fair" run $\run'$ starting in the last configuration of $\run$ whose projection on $q$ is a prefix of $v''_q$ (thus $t_k$ is never released and thus neither are $t_0, \ldots, t_{k-1}$) and whose projection on $p$ is a prefix of $\run_p$ (and thus finite as $\run_p$ tries to acquire $t$, which is never free). As a consequence, $\run\run'$ is a "process-fair" run whose projection on $p$ is finite.
	
	\paragraph{Case 2:} $t_q = t_j$ for some $0 \leq j \leq k$ and $\run_q$ acquires $t_j$ at some point and never releases it. Then we apply the same reasoning as in the previous case for the path $t = t_0 \edge{p_1} \cdots \edge{p_j} t_j$.
	
	\paragraph{Case 3:} $t_q = t_j$ for some $0 \leq j \leq k$ and $t_j$ is used in $v_q$ but not kept indefinitely.
	
	\paragraph{Subcase 3.1:} there is an edge $t' \edge{q} t_j$.
	Then we have a path from $t$ to a cycle $t_j \edge{p_{j+1}} \cdots \edge{p_k} t' \edge{q} t_j$.
	Hence by Lemma~\ref{lem:cond-cycle}, there is a "process-fair" global run with a finite projection on $p$. 
	
	\paragraph{Subcase 3.2:} One of the runs $\run_i$ has a "weak pattern" $\dashover{\set{t_{i-1}}}$. 
	We decompose $\run_i$ as $u_i v_i$ with $u_i$ its largest "neutral" prefix.
	Then we execute $u_i$, then $\run_{i+1} \cdots \run_{k}$. After that we execute a prefix $\run'_q$ of $\run_q$ such that at the end $q$ holds only $t'$, and does not release it later. This prefix exists as $q$ never keeps $t_j$ indefinitely in $\run_q$. We decompose $\run_q$ as $\run'_q \run''_q$. Then we execute $\run_1 \cdots \run_{i-1} \run'_i$. All those runs can be executed as before executing each $\run_{i'}$ both locks of $p_{i'}$ are free, and before executing $v_i$, $t_{i-1}$ is free, which is all that is needed to execute $v_i$ as $\run_i$ has a "weak pattern". Let $\run$ be the run constructed so far.
	Then by Lemma~\ref{lem:fair-exclusive} we can construct a "process-fair" run from the configuration reached by $\run$ whose projection on $q$ is a prefix of $\run''_q$ and whose projection on $p$ is a prefix of $\run_p$.
	As a consequence, $t' = t_k$ is never released in $\run''_q$ and thus neither are $t_0, \ldots, t_{k-1}$. As $\run_p$ tries to take $t = t_0$ at some point, its prefix executed in $\run'$ is finite. 
	Hence $\run \run'$ is a "process-fair" run with a finite projection on $p$.
	
	\paragraph{Subcase 3.3:} There is no edge $t' \edge{q} t_j$ and all $\run_i$ have "strong patterns".
	When executing the $v_q$ part of $\run_q$, $q$ holds a lock at all times, and holds $t_j$ at some point and $t'$ at some point, hence it has to have both at the same time at some moment.
	Hence there is a moment at which $q$ holds one of the locks and is about to get the other. As the system is "exclusive", it means all its available transitions take that lock.
	Hence there is an edge  $t' \edge{q} t_j$ or $t_j \edge{q} t'$ in the graph. As we assumed that there is no edge $t' \edge{q} t_j$, there is one $t_j \edge{q} t'$. 
	Furthermore, as we selected the $\run_i$ so that they had weak patterns whenever possible, it means that for all $i$ there is no run with a weak pattern "witnessing" $t_{i-1} \edge{p_i} t_i$.
	By Lemma~\ref{lem:always-one-weak} this means that there are edges $t_k \edge{p_k} t_{k-1} \edge{p_{k-1}} \cdots \edge{p_{j+1}} t_j$. With the edge $t' \edge{q} t_j$, we obtain a cycle in $G$ with a path from $t$ to it.
	By Lemma~\ref{lem:cond-cycle}, there is a "process-fair" global run with a finite projection on $p$. 
	
	This concludes our case distinction, proving the lemma.	
\end{proof}

\begin{lemma}
	\label{lem:cond-stop}
	If $p$ has a reachable transition acquiring some lock $t$ and there is a path in $G$ from $t$ to some $t'$ such that there is a process $q$ with a local run $\run_q$ with $t' \in \Owns(\run_q)$ and going to a state with no outgoing transitions, then there is a "process-fair" global run with a finite projection on $p$. 
\end{lemma}
\begin{proof}
	Let $s_q$ be the state reached by $\run_q$, we add a self-loop on it with a fresh letter $\#$. As there are no other outgoing transitions from $s_q$ this does not break the exclusiveness. It does not change $G$ either.
	Then $\run_q \#^\omega$ is an infinite run acquiring $t'$ and never releasing it.
	
	Hence by Lemma~\ref{lem:cond-inf}, there is a "process-fair" run $\run$ in this new system whose projection on $p$ is finite. Let $h$ be the morphism such that $h(\#) = \epsilon$ and $h(a) = a$ for all other letters $a$. 
	Then $h(\run)$ is a "process-fair" run of the original system: it is a run as $\#$ does not change the configuration, meaning that all actions of $h(\run)$ can be executed. For the same reason, if a process $p'$ other than $q$ only has finitely many actions in $h(\run)$, then the same is true in $\run$, thus there is a point after which no configuration allows $p'$ to move in $\run$, and thus in $h(\run)$ as well. As for $q$, either it only executes $\#$ from some point on, meaning it has reached $s_q$ and will be immobilised in $h(\run)$, or it never executes any $\#$, in which case $h(\run) = \run$ and it follows the same configurations in both.
\end{proof}



\begin{lemma}\label{lem:exclusiveGraph}
	There is a "process-fair" run whose projection on $p$ is finite if and only if there is a local run $\run_p$ of $p$ leading to a state where all outgoing transitions take some lock $t$ and either 
	
	\begin{enumerate}		
		\item\label{Cx1} $p$ has a local run leading to a state with no outgoing transitions.
		
		\item\label{Cx2} or there is a path from $t$ to a cycle in $G$
		
		
		\item\label{Cx3} or there is a path in $G$ from $t$ to some lock $t'$ and there is a process $q$ with a local run $\run_q$ with an 
		"infinitary pattern" with $t' \in \Owns(\run_q)$. 
	
		
		\item\label{Cx4} or there is a path in $G$ from $t$ to some lock $t'$ and there is a process $q$ with a local run $\run_q$ such that $t' \in \Owns(\run_q)$ and leading to a state with no outgoing transitions.
	\end{enumerate}
\end{lemma}

\begin{proof}
	We start with the left-to-right implication: Say there is a run $\run$ whose projection on $p$ is finite. For each process $p' \in \Proc$ let $\run_{p'}$ be its local run. 
	
	Then $\run_p$ has to end in a state where all available transitions acquire a
	lock $t$. If there are no transitions at all, condition~\ref{Cx1} is
	satisfied. If there is at least one such transition, then $t$ is held
	forever by some other process $p_1$.
	
	We construct a path $t = t_0 \edge{p_0} t_1 \edge{p_1} \cdots$ in $G$ so that all $t_i$ are held indefinitely by some process after some point in the run.
	Say we already constructed those up to $i$.
	
	There is a process $p_{i}$ holding $t_i$ indefinitely.
	If $\run_{p_{i}}$ is infinite, then condition~\ref{Cx3} is satisfied. Otherwise, $\run_{p_{i}}$ is finite, and with a "finitary pattern" such that $t_i \in \Owns(\run_{p_i})$.
	
	If this local run ends up in a state with no outgoing transition then condition~\ref{Cx2} is satisfied, otherwise it must have no choice but to acquire some lock $t'_{i+1}$.
	Hence we construct an infinite path
	$t'_0 \edge{p'_0} t'_1 \edge{p'_1} \cdots$ in $G$.
	
	The set of processes is finite, hence there exist 
	$i < j$ such that $t_i = t_j$, meaning we have reached a cycle. Thus condition~\ref{Cx4} is satisfied.
	
	For the other direction, suppose there exists $t$ as in the statement of the lemma, so that one of the conditions is satisfied.
	
	If condition~\ref{Cx1} is satisfied, then we have a finite run $\run_p$ leading to a state with no outgoing transition. We execute it and then prolong it into a global "process-fair" run by choosing a process uniformly at random and executing one of its available actions if there is any (similarly to the proof of \ref{lem:fair-exclusive}). 
	We obtain a "process-fair" run in which $p$ only has finitely many actions. 
	If condition~\ref{Cx2} is satisfied then we have the result by Lemma~\ref{lem:cond-cycle}.
	If condition~\ref{Cx3} is satisfied then we have the result by Lemma~\ref{lem:cond-stop}.
	If condition~\ref{Cx4} is satisfied then we have the result by Lemma~\ref{lem:cond-inf}.
%	Otherwise we proceed in two steps: first ensure that $t'$ is blocked forever with a finite run $\run$ with actions from a subset of processes $P$, and then use a path from $t$ to $t'$ in $G$ containing no process of $P$ to block $t$ as well.
%	
%	We distinguish cases according to which condition is satisfied for the first step, the second step is common to all cases.
%	
%	If condition~\ref{Cx2} is satisfied, we have a finite run $\run_q$ of some process $q$ such that $t' \in \Owns_q(\run_q)$ and leading to a state with no outgoing transition. We set $\run = \run_q$ and $P = \set{q}$.
%	
%	If condition~\ref{Cx3} is satisfied, then we have an infinite local run $\run_q$ such that eventually $q$ never releases $t'$. We execute a prefix of $\run_q$ up to a point where either:
%	\begin{itemize}
%		\item $q$ holds both of its locks and keeps them indefinitely afterwards.
%		
%		\item or $q$ only holds $t'$ and keeps it forever afterwards.    
%	\end{itemize}
%	We set $\run$ to be that prefix and $P = \set{q}$.
%	
%	If condition~\ref{Cx4} is satisfied, then we execute first the largest prefix $\run^p_k$ of $\run_k$ such that $\Owns_{p_k}(\run_k) = \emptyset$. Then we execute  for each $0 \leq i \leq k-1$ in increasing order the local run $\run^{t_i,t_{i+1}}_{p_i}$ of process $p_i$. Finally we can execute the rest of $\run_k$.
%	This is all possible as before we execute all $\run^{t_i,t_{i+1}}_{p_i}$ (with $i \leq k-1$) $t_i$ and $t_{i+1}$ are free. Furthermore as $\run_k$ has a weak pattern $\dashover{\set{t_k}}$, after executing $\run^p_k$ , the remaining actions only take $t_k$ (which is free at that point) and do nothing else on locks. We set $P = \set{p_1, \ldots, p_k}$ and $\run$ as the run described above.
%	
%	In all cases we have a finite run of processes of $P$ leading to a configuration where all locks that are not free will never be released, and $t'$ is one of them. Let $\Theta$ be the set of non-free locks after executing $\run$.
%	
%	Then let $t = t'_0 \edge{p'_0} \cdots \edge{p'_{n-1}} t'_n$ be a path in $G$ of minimal length from $t$ to some $t_n \in \Theta$. It exists as there is a path from $t$ to $t' \in \Theta$ in $G$.  All locks are free at the start, hence we can execute (in increasing order) for each $i$ the local run $\run_{p'_i}^{t'_i, t'_{i+1}}$. As we took a shortest path, no $t'_i$ is in $\Theta$.
%	
%	After we do that, we execute $t'$ 
\end{proof}


	To conclude the proof of Proposition~\ref{prop:ptime-exclusive}, by Lemma~\ref{lem:exclusiveGraph}, we only have to check the four conditions listed in its statement.	
	Here is our algorithm: 
	
	We start by looking, in the transition system of process $p$, for a reachable local state with no outgoing transition. If there is one, we accept.

	Then we compute all pairs $(q, t)$ such that either there is an infinite run of process $q$ keeping $t$ indefinitely from some point on or there is a run $\run_q$ with $t \in \Owns(\run_q)$ leading to a state with no outgoing transitions. 
	As our system is "sound", the set of locks a process has is determined by its state. Let $\ownfunc_p$ be the function described in Definition~\ref{def:soundness}.
	Then we compute all pairs $(t, t')$ such that some process $p'$ has a reachable state $s$ with $\ownfunc_{p'}(s) = \set{t}$ and all outgoing transitions of $s$ acquiring $t'$.
	We obtain the edges of $G$.
	
	For both locks of $p'$, we check that there is a reachable transition acquiring it, and there is a path in $G$ to either a cycle or to a $t$ from one of the pairs $(q,t)$ computed above. If it is the case for one of them, we accept, otherwise we reject.
	This can all be done in polynomial time, proving the proposition.

==> Stair-dec.tex <==
\section{Proof of Lemma~\ref{lem:stair-dec}}
\label{sec:stair}

\STAIR*

\begin{proof}
	Let $\run$ be a local run of some process $p$. 
	We start by decomposing it as 
	\[\run=\run_0 a_1 \run_1 a_2 \cdots \run_{k-1} a_k \run_{\infty}\]
	with $a_1, \ldots, a_k$ the actions getting a lock that is not released later
	in the run. 
	For all $i$ let $t_i$ be the lock taken by $a_i$,  namely $op(a_i) = \get{t_i}$.
	
	We check that all $\run_0,\dots,\run_{k-1}$ are "neutral". Consider some $\run_i$. 
	If a lock $t$ is taken in $\run_i$ then it must be released later in the run
	because $a_{i+1}$ is the next operation that takes a lock and does not release
	it.
	But because of the nesting discipline $t$ cannot be released after $a_{i+1}$. 
	So it must be released in $\run_i$.
	
	% As the system is "nested", a lock acquired before an $a_i$ cannot be released afterwards: this would require $t_i$ to be released after $a_i$, which never happens.
	% Hence for all $i$ after executing $\run_0 a_1 \run_1 a_2 \cdots \run_{i-1}$ (right before executing $a_i$), $p$ holds locks $\set{t_1, \ldots, t_{i-1}}$.
	% Thus after executing $\run_0 a_1 \run_1 a_2 \cdots \run_{i-1} a_i$, $p$ holds locks $\set{t_1, \ldots, t_{i}}$.
	
	% Therefore before and after executing each $\run_i$ process $p$ holds the same locks, hence it is neutral.
	
	Now we look at $\run_\infty$. Every lock acquired in it must be
	released eventually. 
	Thus if the run is finite we can set $\run_{k} =\run_{\infty}$ and $\run_i=\epsilon$ for all $i \geq k+1$.
	
	If the run is infinite then we proceed as follows: 
	Before executing $\run_\infty$, $p$ holds $t_1, \ldots, t_k$.
	We construct a sequence of "neutral" runs $\run'_j$ such that $\run_\infty = \run'_{1} \run'_2 \cdots$.
	Say we constructed $\run'_1 \cdots \run'_j$.
	As they are all "neutral", after executing them $p$ holds $t_1, \ldots, t_k$.
	The next action $a$ in $\run_\infty$ cannot release a lock as none of those locks are ever released.
	If $a$ does not get a lock then we can simply set $\run_{j+1} = a$.
	If $a$ acquires lock $t$ then let $\run_{j+1}$ be the infix of $\run_\infty$
	starting with $a$ and ending with the next action releasing $t$. 
	This run is "neutral" as the system is "nested".
	Then let $j$ be such that $\run'_{1} \cdots \run'_{j}$ contains all $\get{t}$ operations with $t$ acquired finitely many times in $\run_{\infty}$.
	We set $\run_{k} = \run'_{1} \cdots \run'_{j}$ and for all $i \geq k+1$, $\run_i = \run'_{j-k+i}$. We obtain our decomposition.
\end{proof}
